CLIMATELI: Evaluating Entity Linking on Climate Change Data

Climate Change (CC) is a pressing topic of global importance, attracting increasing attention across research fields, from social sciences to Natural Language Processing (NLP). CC is also discussed in various settings and communication platforms, from academic publications to social media forums. Understanding who and what is mentioned in such data is a first critical step to gaining new insights into CC. We present CLIMATELI (CLIMATe Entity LInking), the first manually annotated CC dataset that links 3,087 entity spans to Wikipedia. Using CLIMATELI (CLIMATe Entity LInking), we evaluate existing entity linking (EL) systems on the CC topic across various genres and propose automated filtering methods for CC entities. We find that the performance of EL models notably lags behind humans at both token and entity levels. Testing within the scope of retaining or excluding non-nominal and/or non-CC entities particularly impacts the models' performances.

==> backup.tex <==


\paragraph{CC \& Event extraction}
\begin{itemize}
\item \citet{nakshatri-etal-2023-using} extracts event-focused clusters on issues such as Climate Change and Abortion, but without entity linking.

\end{itemize}

\paragraph{CC \& other NLP tasks}
\begin{itemize}
\item \item CC Question Answering dataset \citep{rony_climate_2022}
\item 
\end{itemize}

\paragraph{Other EL}
\begin{itemize}
\item 
\citet{sorokin-gurevych-2018-mixing}: applying EL KB to QA
\item 

\end{itemize}

==> tables/5_genres.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{llcccc|cccc}
\toprule
\multicolumn{1}{l}{}      & \multicolumn{1}{l}{} & \multicolumn{4}{c}{typed}     & \multicolumn{4}{c}{untyped}   \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & accuracy & precision & recall & f1 & accuracy & precision & recall & f1 \\ \midrule
\multirow{5}{*}{GENRE}    & academic             & 66.77 & 44.62 & 17.10 & 24.72 & 70.15 & 54.58 & 20.92 & 30.24 \\
      & ipcc                 & 61.91 & \textbf{49.73} & 11.66 & 18.89 & 64.68 & \textbf{68.11} & 15.97 & 25.87 \\
      & news                 & 74.70 & 45.61 & 25.39 & 32.62 & 77.64 & 57.89 & 32.23 & \textbf{41.41} \\
      & vlog                 & \textbf{78.53} & 45.51 & \textbf{31.40} & \textbf{37.16} & \textbf{79.86} & 50.60 & \textbf{34.92} & 41.32 \\
      & wiki                 & 68.80 & 43.60 & 23.18 & 30.27 & 72.41 & 53.78 & 28.59 & 37.34 \\ \midrule
\multirow{5}{*}{TagMe}    & academic             & 55.01 & 13.81 & 19.08 & 16.03 & 76.63 & 47.62 & 65.80 & 55.26 \\
      & ipcc                 & 53.80 & 18.30 & 19.39 & 18.83 & \textbf{77.45} & \textbf{60.17} & 63.75 & \textbf{61.91} \\
      & news                 & 58.25 & 16.92 & 27.93 & 21.08 & 74.58 & 41.66 & \textbf{68.75} & 51.88 \\
      & vlog                 & \textbf{63.24} & \textbf{18.67} & \textbf{28.51} & \textbf{22.57} & 72.37 & 40.19 & 61.36 & 48.57 \\
      & wiki                 & 55.03 & 15.12 & 19.63 & 17.08 & 75.87 & 48.10 & 62.44 & 54.34 \\ \midrule
\multirow{5}{*}{Wikifier} & academic             & 69.52 & 42.16 & \textbf{65.65} & 51.34 & 75.29 & 50.29 & 78.32 & 61.25 \\
      & ipcc                 & \textbf{70.52} & \textbf{48.62} & 60.33 & \textbf{53.85} & \textbf{79.92} & \textbf{60.67} & 75.29 & \textbf{67.19} \\
      & news                 & 68.44 & 33.70 & 60.55 & 43.30 & 74.58 & 42.50 & 76.37 & 54.61 \\
      & vlog                 & 69.32 & 31.00 & 60.33 & 40.95 & 75.53 & 43.10 & \textbf{83.88} & 56.94 \\
      & wiki                 & 65.67 & 35.55 & 52.86 & 42.51 & 75.10 & 50.52 & 75.12 & 60.41 \\
\bottomrule
\end{tabular} 
}
\caption{Typed and untyped token-level accuracy and entity-level  precision, recall, and F1
scores of GENRE, TagMe and Wikifier models on 5 genres documents (on all annotations).}
\label{fig:5_genres}
\end{table*}

==> tables/all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{clllllllll}
\toprule
\multicolumn{1}{l}{}       &     & \multicolumn{4}{c}{typed}     & \multicolumn{4}{c}{untyped}   \\
\multicolumn{1}{l}{} &
&
\multicolumn{1}{c}{token-level} &
\multicolumn{3}{c}{entity-level} &
\multicolumn{1}{c}{token-level} &
\multicolumn{3}{c}{entity-level} \\
\multicolumn{1}{l}{} &
&
\multicolumn{1}{c}{accuracy} &
\multicolumn{1}{c}{precision} &
\multicolumn{1}{c}{recall} &
\multicolumn{1}{c}{F1} &
\multicolumn{1}{c}{accuracy} &
\multicolumn{1}{c}{precision} &
\multicolumn{1}{c}{recall} &
\multicolumn{1}{c}{F1} \\ \midrule
\multicolumn{2}{c}{GENRE}        & 70.15 & 45.46 & 20.60 & 28.35 & 72.98 & 55.90 & 25.33 & 34.86 \\ \midrule
\multirow{10}{*}{TagMe}    & 0.1 & 64.43 & 33.33 & 0.03  & 0.06  & 64.47 & 66.67 & 0.06  & 0.13  \\
& 0.2 & 64.43 & 10.00 & 0.03  & 0.06  & 64.57 & 40.00 & 0.13  & 0.26  \\
& 0.3 & 64.46 & 21.74 & 0.16  & 0.32  & 64.75 & 69.57 & 0.52  & 1.03  \\
& 0.4 & 64.57 & 32.73 & 0.58  & 1.15  & 65.08 & 65.45 & 1.17  & 2.29  \\
& 0.5 & 64.74 & 29.58 & 1.36  & 2.60  & 66.12 & 66.20 & 3.05  & 5.82  \\
& 0.6 & 64.87 & 23.08 & 2.33  & 4.24  & 67.97 & 62.50 & 6.32  & 11.47 \\
& 0.7 & 65.40 & 24.48 & 5.34  & 8.77  & 71.20 & 64.54 & 14.09 & 23.13 \\
& 0.8 & 65.82 & 24.91 & 11.27 & 15.52 & 75.25 & 62.78 & 28.41 & 39.12 \\
& 0.9 & 63.99 & 21.46 & 17.82 & 19.47 & 77.64 & 56.15 & 46.61 & 50.94 \\
& 1.0 & 57.03 & 16.47 & 22.22 & 18.92 & 75.39 & 47.71 & 64.37 & 54.80 \\ \midrule
\multirow{10}{*}{Wikifier} & 0.1 & 64.51 & 37.50 & 0.19  & 0.39  & 64.55 & 50.00 & 0.26  & 0.52  \\
& 0.2 & 65.19 & 53.54 & 1.72  & 3.33  & 65.46 & 57.58 & 1.85  & 3.58  \\
& 0.3 & 66.02 & 53.42 & 4.05  & 7.53  & 66.63 & 61.97 & 4.70  & 8.73  \\
& 0.4 & 67.42 & 53.50 & 7.42  & 13.03 & 68.55 & 65.65 & 9.10  & 15.99 \\
& 0.5 & 69.37 & 57.77 & 11.44 & 19.09 & 70.79 & 68.58 & 13.57 & 22.66 \\
& 0.6 & 71.36 & 60.49 & 15.97 & 25.27 & 73.03 & 69.08 & 18.24 & 28.86 \\
& 0.7 & 73.36 & 61.36 & 21.70 & 32.07 & 75.39 & 70.15 & 24.81 & 36.66 \\
& 0.8 & 75.33 & 59.25 & 29.06 & 38.99 & 78.38 & 69.62 & 34.14 & 45.82 \\
& 0.9 & 76.94 & 56.12 & 38.94 & 45.97 & 81.04 & 67.51 & 46.84 & 55.31 \\
& 1.0 & 68.64 & 38.36 & 59.93 & 46.78 & 76.02 & 49.55 & 77.42 & 60.43\\
\bottomrule
\end{tabular}
\caption{Typed and untyped token-level accuracy and entity-level  precision, recall, and F1
scores of GENRE, TagMe and Wikifier models annotations (on all annotations).}
\label{tab:all}
\end{table*}

==> tables/c_only.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{clllllllll}
\toprule
\multicolumn{1}{l}{}       &     & \multicolumn{4}{c}{typed}     & \multicolumn{4}{c}{untyped}   \\
\multicolumn{1}{l}{} &
&
\multicolumn{1}{c}{token-level} &
\multicolumn{3}{c}{entity-level} &
\multicolumn{1}{c}{token-level} &
\multicolumn{3}{c}{entity-level} \\
\multicolumn{1}{l}{} &
&
\multicolumn{1}{c}{accuracy} &
\multicolumn{1}{c}{precision} &
\multicolumn{1}{c}{recall} &
\multicolumn{1}{c}{F1} &
\multicolumn{1}{c}{accuracy} &
\multicolumn{1}{c}{precision} &
\multicolumn{1}{c}{recall} &
\multicolumn{1}{c}{F1} \\ \midrule
\multicolumn{2}{c}{GENRE}        & 82.14 & 50.56 & 26.98 & 35.19 & 84.12 & 58.34 & 31.13 & 40.60 \\ \midrule
\multirow{10}{*}{TagMe}    & 0.1 & 76.55 & 0.00  & 0.00  & 0.00  & 76.59 & 50.00 & 0.05  & 0.11  \\
& 0.2 & 76.55 & 0.00  & 0.00  & 0.00  & 76.68 & 37.50 & 0.16  & 0.33  \\
& 0.3 & 76.57 & 20.00 & 0.22  & 0.43  & 76.82 & 70.00 & 0.76  & 1.51  \\
& 0.4 & 76.65 & 33.33 & 0.87  & 1.70  & 77.13 & 68.75 & 1.80  & 3.51  \\
& 0.5 & 76.86 & 31.45 & 2.13  & 3.99  & 77.98 & 68.55 & 4.64  & 8.70  \\
& 0.6 & 77.00 & 23.75 & 3.39  & 5.93  & 79.43 & 63.98 & 9.12  & 15.97 \\
& 0.7 & 77.50 & 25.81 & 7.86  & 12.06 & 82.04 & 65.41 & 19.93 & 30.56 \\
& 0.8 & 77.81 & 25.91 & 14.04 & 18.21 & 84.40 & 62.40 & 33.81 & 43.85 \\
& 0.9 & 77.45 & 24.36 & 20.43 & 22.22 & 86.24 & 57.72 & 48.39 & 52.64 \\
& 1.0 & 76.61 & 22.13 & 22.67 & 22.40 & 86.73 & 54.35 & 55.65 & 54.99 \\ \midrule
\multirow{10}{*}{Wikifier} & 0.1 & 76.59 & 38.46 & 0.27  & 0.54  & 76.63 & 53.85 & 0.38  & 0.76  \\
& 0.2 & 77.22 & 54.17 & 2.84  & 5.40  & 77.48 & 58.33 & 3.06  & 5.81  \\
& 0.3 & 77.83 & 51.47 & 5.73  & 10.32 & 78.41 & 60.29 & 6.72  & 12.09 \\
& 0.4 & 79.10 & 53.54 & 11.14 & 18.44 & 80.09 & 63.78 & 13.27 & 21.97 \\
& 0.5 & 80.80 & 58.08 & 17.48 & 26.87 & 81.89 & 66.42 & 19.99 & 30.73 \\
& 0.6 & 82.43 & 60.87 & 24.47 & 34.90 & 83.74 & 67.66 & 27.20 & 38.80 \\
& 0.7 & 84.21 & 61.92 & 33.75 & 43.69 & 85.69 & 68.24 & 37.19 & 48.14 \\
& 0.8 & 85.33 & 58.94 & 43.20 & 49.86 & 87.34 & 65.87 & 48.28 & 55.72 \\
& 0.9 & 86.02 & 56.75 & 51.67 & 54.09 & 88.45 & 64.31 & 58.55 & 61.29 \\
& 1.0 & 84.96 & 51.63 & 57.24 & 54.29 & 87.92 & 60.20 & 66.74 & 63.30\\
\bottomrule
\end{tabular}
\caption{Typed and untyped token-level accuracy and entity-level  precision, recall, and F1
scores of GENRE, TagMe and Wikifier models annotations (on climate change related annotations).}
\label{tab:c_only}
\end{table*}

==> tables/entities_length.tex <==
\begin{table}[]
\centering
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
&  academic & ipcc & news & vlog & wiki \\
All  & 1.91 & 1.85 & 1.80 & 1.72 & 1.79 \\
N-only & 1.99  & 1.92 & 1.88 & 1.80 & 1.88 \\
C-only & 2.10  & 2.00 & 1.94 & 1.88 & 1.97 \\
NC-only &  2.13 & 2.04 & 2.00 & 1.93 & 2.03 \\ \bottomrule
\end{tabular}
}
\caption{Average number of tokens per entity in human annotations of document in genre academic, ipcc, news, vlog, wiki.}
\label{tab:length}
\end{table}

==> tables/n_only.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{clllllllll}
\toprule
\multicolumn{1}{l}{}       &     & \multicolumn{4}{c}{typed}     & \multicolumn{4}{c}{untyped}   \\
\multicolumn{1}{l}{} &
&
\multicolumn{1}{c}{token-level} &
\multicolumn{3}{c}{entity-level} &
\multicolumn{1}{c}{token-level} &
\multicolumn{3}{c}{entity-level} \\
\multicolumn{1}{l}{} &
&
\multicolumn{1}{c}{accuracy} &
\multicolumn{1}{c}{precision} &
\multicolumn{1}{c}{recall} &
\multicolumn{1}{c}{F1} &
\multicolumn{1}{c}{accuracy} &
\multicolumn{1}{c}{precision} &
\multicolumn{1}{c}{recall} &
\multicolumn{1}{c}{F1} \\ \midrule
\multicolumn{2}{c}{GENRE}        & 77.67 & 53.35 & 25.15 & 34.18 & 79.94 & 63.56 & 29.97 & 40.73 \\ \midrule
\multirow{10}{*}{TagMe}    & 0.1 & 71.00 & 33.33 & 0.04  & 0.09  & 71.04 & 66.67 & 0.09  & 0.17  \\
& 0.2 & 71.00 & 10.00 & 0.04  & 0.08  & 71.14 & 40.00 & 0.17  & 0.34  \\
& 0.3 & 71.01 & 21.74 & 0.21  & 0.42  & 71.29 & 69.57 & 0.68  & 1.35  \\
& 0.4 & 71.11 & 31.48 & 0.72  & 1.42  & 71.61 & 64.81 & 1.49  & 2.92  \\
& 0.5 & 71.31 & 29.85 & 1.71  & 3.23  & 72.50 & 64.93 & 3.71  & 7.02  \\
& 0.6 & 71.47 & 23.81 & 2.98  & 5.30  & 74.18 & 62.93 & 7.89  & 14.02 \\
& 0.7 & 72.01 & 25.04 & 6.56  & 10.40 & 77.14 & 65.69 & 17.22 & 27.29 \\
& 0.8 & 72.56 & 25.23 & 12.62 & 16.82 & 80.51 & 64.54 & 32.27 & 43.02 \\
& 0.9 & 72.23 & 23.21 & 19.44 & 21.16 & 83.53 & 61.48 & 51.49 & 56.04 \\
& 1.0 & 70.30 & 20.12 & 23.70 & 21.76 & 84.82 & 57.20 & 67.39 & 61.88 \\ \midrule
\multirow{10}{*}{Wikifier} & 0.1 & 71.07 & 37.50 & 0.26  & 0.51  & 71.12 & 50.00 & 0.34  & 0.68  \\
& 0.2 & 71.71 & 54.64 & 2.26  & 4.34  & 71.96 & 58.76 & 2.43  & 4.67  \\
& 0.3 & 72.46 & 53.95 & 5.24  & 9.56  & 73.04 & 62.72 & 6.10  & 11.11 \\
& 0.4 & 73.74 & 54.50 & 9.55  & 16.25 & 74.80 & 66.67 & 11.68 & 19.88 \\
& 0.5 & 75.51 & 58.41 & 14.07 & 22.67 & 76.73 & 69.38 & 16.71 & 26.93 \\
& 0.6 & 77.36 & 61.02 & 19.82 & 29.92 & 78.80 & 69.69 & 22.63 & 34.17 \\
& 0.7 & 79.17 & 62.50 & 26.64 & 37.36 & 80.84 & 71.20 & 30.35 & 42.56 \\
& 0.8 & 80.97 & 60.57 & 34.44 & 43.91 & 83.46 & 71.29 & 40.54 & 51.68 \\
& 0.9 & 82.59 & 59.38 & 43.86 & 50.45 & 85.84 & 71.73 & 52.98 & 60.95 \\
& 1.0 & 82.67 & 52.34 & 57.72 & 54.90 & 87.95 & 68.07 & 75.06 & 71.40\\
\bottomrule
\end{tabular}
\caption{Typed and untyped token-level accuracy and entity-level  precision, recall, and F1
scores of GENRE, TagMe and Wikifier models annotations (only on nominal annotations).}
\label{tab:all}
\end{table*}

==> tables/nc_only.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{clllllllll}
\toprule
\multicolumn{1}{l}{}       &     & \multicolumn{4}{c}{typed}     & \multicolumn{4}{c}{untyped}   \\
\multicolumn{1}{l}{} &
&
\multicolumn{1}{c}{token-level} &
\multicolumn{3}{c}{entity-level} &
\multicolumn{1}{c}{token-level} &
\multicolumn{3}{c}{entity-level} \\
\multicolumn{1}{l}{} &
&
\multicolumn{1}{c}{accuracy} &
\multicolumn{1}{c}{precision} &
\multicolumn{1}{c}{recall} &
\multicolumn{1}{c}{F1} &
\multicolumn{1}{c}{accuracy} &
\multicolumn{1}{c}{precision} &
\multicolumn{1}{c}{recall} &
\multicolumn{1}{c}{F1} \\ \midrule
\multicolumn{2}{c}{GENRE}        & 84.09 & 52.90 & 29.89 & 38.20 & 85.92 & 60.71 & 34.30 & 43.84 \\ \midrule
\multirow{10}{*}{TagMe}    & 0.1 & 78.50 & 0.00  & 0.00  & 0.00  & 78.54 & 50.00 & 0.06  & 0.13  \\
& 0.2 & 78.50 & 0.00  & 0.00  & 0.00  & 78.64 & 37.50 & 0.19  & 0.38  \\
& 0.3 & 78.52 & 20.00 & 0.25  & 0.50  & 78.78 & 70.00 & 0.88  & 1.74  \\
& 0.4 & 78.60 & 33.33 & 1.01  & 1.96  & 79.08 & 68.75 & 2.08  & 4.04  \\
& 0.5 & 78.81 & 31.97 & 2.46  & 4.57  & 79.92 & 68.03 & 5.23  & 9.72  \\
& 0.6 & 78.96 & 24.51 & 3.91  & 6.74  & 81.35 & 64.43 & 10.28 & 17.73 \\
& 0.7 & 79.44 & 25.75 & 8.64  & 12.94 & 83.89 & 65.98 & 22.13 & 33.14 \\
& 0.8 & 79.75 & 25.50 & 14.50 & 18.49 & 86.07 & 63.41 & 36.07 & 45.98 \\
& 0.9 & 79.71 & 24.81 & 20.81 & 22.63 & 87.99 & 60.75 & 50.95 & 55.42 \\
& 1.0 & 79.43 & 23.31 & 22.89 & 23.10 & 88.88 & 58.83 & 57.76 & 58.29 \\ \midrule
\multirow{10}{*}{Wikifier} & 0.1 & 78.54 & 38.46 & 0.32  & 0.63  & 78.58 & 53.85 & 0.44  & 0.88  \\
& 0.2 & 79.18 & 55.32 & 3.28  & 6.19  & 79.42 & 59.57 & 3.53  & 6.67  \\
& 0.3 & 79.76 & 52.00 & 6.56  & 11.65 & 80.31 & 61.00 & 7.69  & 13.66 \\
& 0.4 & 80.98 & 54.64 & 12.61 & 20.49 & 81.92 & 64.75 & 14.94 & 24.28 \\
& 0.5 & 82.61 & 58.78 & 18.79 & 28.48 & 83.64 & 67.06 & 21.44 & 32.49 \\
& 0.6 & 84.21 & 61.28 & 26.54 & 37.04 & 85.46 & 67.98 & 29.45 & 41.09 \\
& 0.7 & 85.83 & 62.87 & 36.19 & 45.94 & 87.20 & 69.22 & 39.85 & 50.58 \\
& 0.8 & 86.97 & 60.29 & 44.89 & 51.46 & 88.82 & 67.57 & 50.32 & 57.68 \\
& 0.9 & 87.87 & 59.89 & 53.09 & 56.28 & 90.08 & 68.28 & 60.53 & 64.17 \\
& 1.0 & 87.62 & 57.79 & 56.62 & 57.20 & 90.27 & 68.02 & 66.65 & 67.32\\
\bottomrule
\end{tabular}
\caption{Typed and untyped token-level accuracy and entity-level  precision, recall, and F1
scores of GENRE, TagMe and Wikifier models annotations (on all annotations).}
\label{tab:all}
\end{table*}
